Code Change Intention, Development Artifact and History Vulnerability: Putting Them Together for Vulnerability Fix Detection by LLM

Detecting vulnerability fix commits in open-source software is crucial for maintaining software security. To help OSS identify vulnerability fix commits, several automated approaches are developed. However, existing approaches like VulFixMiner and CoLeFunDa, focus solely on code changes, neglecting essential context from development artifacts. Tools like Vulcurator, which integrates issue reports, fail to leverage semantic associations between different development artifacts (e.g., pull requests and history vulnerability fixes). Moreover, they miss vulnerability fixes in tangled commits and lack explanations, limiting practical use. Hence to address those limitations, we propose LLM4VFD, a novel framework that leverages Large Language Models (LLMs) enhanced with Chain-of-Thought reasoning and In-Context Learning to improve the accuracy of vulnerability fix detection. LLM4VFD comprises three components: (1) Code Change Intention, which analyzes commit summaries, purposes, and implications using Chain-of-Thought reasoning; (2) Development Artifact, which incorporates context from related issue reports and pull requests; (3) Historical Vulnerability, which retrieves similar past vulnerability fixes to enrich context. More importantly, on top of the prediction, LLM4VFD also provides a detailed analysis and explanation to help security experts understand the rationale behind the decision. We evaluated LLM4VFD against state-of-the-art techniques, including Pre-trained Language Model-based approaches and vanilla LLMs, using a newly collected dataset, BigVulFixes. Experimental results demonstrate that LLM4VFD significantly outperforms the best-performed existing approach by 68.1%--145.4%. Furthermore, We conducted a user study with security experts, showing that the analysis generated by LLM4VFD improves the efficiency of vulnerability fix identification.

==> components/08-related-work.tex <==
\section{Related Work}
In this section, we present the related work of our paper. We focus on the research directly focusing on vulnerability fix detection and the recent LLM adoptions in software engineering focusing on vulnerability related tasks.


\subsection{LLM in Vulnerability Management}

In various software engineering challenges related to vulnerability, researchers have explored using LLM to complete the tasks~\cite{hou2023large}.
%
Compared to other machine learning techniques such as deeping learning, LLM shows superior capability is tasks involving code understanding~\cite{shen2022benchmarking} (\eg code summary~\cite{wang2023codet5+} and code generation~\cite{bareiss2022code,gilbert2023semantic,jiang2023selfevolve,liu2024your}) and overcomes many limitations of previous techniques~\cite{wu2023effective,hou2023large}.
The strength of LLM leads to researchers adopting the tool in vulnerability related tasks.
To our best knowledge, we are the first work in leveraging LLM on the vulnerability fix detection task.
Previous works mainly focused on vulnerability detection and vulnerability fix~\cite{zhou2024large}.

\subsubsection{Vulnerability Detection}
\citet{chan2023transformer} proposed a system based on vulnerable code patterns to detect vulnerabilities on code.
\citet{chen2023diversevul} created a dataset for vulnerable source code and compared the performance of deep learning models and LLM models on the dataset. Their results shows promising results in LLM models.
\citet{thapa2022transformer} researched LLM's performance of C/C++ source codes with multiple vulnerabilities.
\citet{cheng2024llm} presented an approach Vercation to identify vulnerable versions of C/C++ open-source software.
\citet{du2024vul} proposed Vul-RAG a framework that first constructs a vulnerability knowledge base than extract knowledge from CVE instances. The framework is then able to predict whether a given code snippet is vulnerable based on a RAG system that retrieves from the knowledge base.


\subsubsection{Vulnerability Repair\xy{remove if need space}}
\citet{pearce2023examining} explored the LLM's ability on zero-shot vulnerability repair and demonstrated that while each vulnerability can be repaired by a LLM, no single LLM can successfully fix all vulnerabilities.
\citet{islam2024llm} proposed CodeGen2 to generate vulnerability fixes based on code comment.
\citet{kulsum2024case} introduced a technique VRpilot that leverages CoT to reason about vulnerability and generates patch candidates for fixes.
\citet{zhang2024evaluating} evaluated the performance of LLM in fixing memory corruption vulnerabilities in real-world C/C++ code.
\citet{nong2024automated} proposed LLMPATCH which leverages adaptive prompting to create patches for vulnerabilities.

